Dueling Bandits with Qualitative Feedback

We formulate and study a novel multi-armed bandit problem called the qualitative dueling bandit (QDB) problem, where an agent observes not numeric but qualitative feedback by pulling each arm. We employ the same regret as the dueling bandit (DB) problem where the duel is carried out by comparing the qualitative feedback. Although we can naively use classic DB algorithms for solving the QDB problem, this reduction significantly worsens the performance---actually, in the QDB problem, the probability that one arm wins the duel over another arm can be directly estimated without carrying out actual duels. In this paper, we propose such direct algorithms for the QDB problem. Our theoretical analysis shows that the proposed algorithms significantly outperform DB algorithms by incorporating the qualitative feedback, and experimental results also demonstrate vast improvement over the existing DB algorithms.

==> Experiments/Synthetic_Setting.tex <==
%As proved in Theorem~\ref{thm:thompson-fails-borda}, Thompson Borda sampling can incur the polynomial regret. We confirm this phenomenon through experiments as well. In We run Thompson Borda sampling and UCB-Borda in the setting that Thompson Borda sampling is suggested to have the polynomial regret in Appendix~\ref{sec:Proof-of-thompson-fails-borda}, in which we have $K=3$ arms and each feedback distribution is  \label{eq:thompson-fails-distributions}
%\begin{align*}
%\vecarm{P}{1} &= ( 0.01,  0.01,  0.96,  0.01,  0.01)^\top,\\
%\vecarm{P}{2} &= (0.01,  0.26,  0.46,  0.26,  0.01)^\top,\\
%\vecarm{P}{3} &= (0.5 ,  0.25,  0.01,  0.23,  0.01)^\top,
%\end{align*}
Theorem~\ref{thm:thompson-fails-borda} suggests that Thompson Borda sampling can incur the polynomial regret, which we confirm through experiments. In the proof of Theorem~\ref{thm:thompson-fails-borda} in Appendix~\ref{sec:Proof-of-thompson-fails-borda}, we consider the feedback distributions \eqref{eq:thompson-fails-distributions} which causes the polynomial regret. We run Thompson Borda sampling and UCB-Borda in a such instance, where the hyper-paramter $\varepsilon$ in  \eqref{eq:thompson-fails-distributions} is set $\varepsilon=0.01$.

\begin{figure}
    \centering
    \includegraphics[width = 0.7\linewidth]{fig/Thompson_fails_2.pdf}
    \caption{The regret of proposed algorithms in the instance that Thompson Borda sampling suffers the polynomial regret.}
    \label{fig:Thompson-fails}
\end{figure}

Figure~\ref{fig:Thompson-fails} is the log-log plot of the regrets of both algorithms. As suggested in Theorem~\ref{thm:thompson-fails-borda}, Thompson Borda sampling suffers from polynomial regret after we have enough rounds ($t > 10^6$), while Borda-UCB shows sub-polynomial increase around $t=10^8$. Therefore, we can expect that eventually, Borda-UCB performs better than Thompson Borda sampling with larger $T$.

However, Thompson Borda sampling performs surprisingly well when the number of rounds is moderate. This is because Thompson Borda sampling explores less than necessary. As discussed in Appendix~\ref{sec:Proof-of-thompson-fails-borda}, in this setting, the agent has to accurately estimate $\vecarm{P}{3}$ in order to determine the Borda winner, though pulling arm 3 incurs a large regret. Therefore, UCB-Borda suffers from this large exploration costs, while Thompson Borda sampling exploits arms~1 and~2, which avoid paying much cost for the exploration.


==> Lemma/Condorcet_pulled.tex <==
\begin{lem}\label{lem:Condorcet_pulled}
	\begin{align*}
		&\prob{a_t \neq a^*_\Condorcet, N_{a^*_\Condorcet}(t) \leq n} \\
		&\quad \leq (2^L+C_1)Kt^K\exp\left(-\frac{t-n}{K}\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right)
	\end{align*}
\end{lem}

==> Lemma/Dirichlet_tail_bound.tex <==
\begin{lem}\label{lem:Dirichlet-tail-bound}
    Let $\tilde{\vec{P}}$ be a sample drawn from Dirichlet distribution $\Dir(nP_1+1,\dots,nP_L+1)$ for $n>0$ and  $\vec{P} = (P_1,\dots,P_L)\in\mathcal{D}_L$,.
    For all $\vec{P}'=P'_1,\dots,P'_L)\in \mathcal{D}_L$, we have
    \begin{align*}
        &\prob{\tilde{P}_1 \leq P'_1, \dots, \tilde{P}_{L-1} \leq P'_{L-1}, \tilde{P}_{L} \geq P'_L} \\
         &\quad \geq \frac{(P'_L)^{L-1}}{\mathrm{e}^{L/6}C_1}(n+L)^{-\frac{L-1}{2}}\exp(-n \KL{\vec{P}}{\vec{P}'})
    \end{align*}
    for $C_1$ defined in \eqref{eq:c_1-def}.
\end{lem}

\begin{proof}
From the probability density function of Dirichlet distribution, we have
    \begin{align}
        &\prob{\tilde{P}_1 \leq P'_1, \dots, \tilde{P}_{L-1} \leq P'_{L-1}, \tilde{P}_{L} \geq P'_L} \\
         &= \frac{\Gamma(n+L)}{\prod_{i=1}^L \Gamma(nP_i + 1)}\\
         &\quad   \int_0^{P'_1} \intd x_1\cdots\int_0^{P'_{L-1}} \intd x_{L-1} \left(1-\sum_{i=1}^{L-1} x_i\right)^{nP_L}\prod_{i=1}^{L-1} x_i^{nP_i}\\
         &= \frac{\Gamma(n+L)}{\prod_{i=1}^L \Gamma(nP_i + 1)}  \int_0^{P'_2} \intd x_2\cdots\int_0^{P'_{L-1}} \intd x_{L-1} \prod_{i=2}^{L-1} x_i^{nP_i}\\
         &\quad ~~~~~~~~~~  \int_0^{P'_1} x^{nP_1}_1\left(1-\sum_{i=1}^{L-1} x_i\right)^{nP_L} \intd x_1 \\
         &\geq \frac{\Gamma(n+L)}{\prod_{i=1}^L \Gamma(nP_i + 1)}  \int_0^{P'_2} \intd x_2\cdots\int_0^{P'_{L-1}} \intd x_{L-1} \prod_{i=2}^{L-1} x_i^{nP_i}\\
         &\quad~~~~~~~~~~ \left[x_1^{nP_1} \left( -\frac{\left(1-\sum_{i=1}^{L-1} x\right)^{nP_L+1}}{nP_L+1}\right)\right]_0^{P'_1}\\
         &= \frac{\Gamma(n+L)}{\prod_{i=1}^L \Gamma(nP_i + 1)}\frac{(P'_1)^{nP_1}}{nP_L+1}  \int_0^{P'_2} \intd x_2\cdots\int_0^{P'_{L-1}} \intd x_{L-1} \\
         &\quad ~~~~~~~~~~ \left(1-P'_1-\sum_{i=2}^{L-1} x_i\right)^{nP_L+1}\prod_{i=2}^{L-1} x_i^{nP_i}.
    \end{align}
The inequality holds for integration by parts.  By repeating this calculation, we have
	\begin{align}
		&\prob{\tilde{P}_1 \leq P'_1, \dots, \tilde{P}_{L-1} \leq P'_{L-1}, \tilde{P}_{L} \geq P'_L} \\
		&\geq \frac{\Gamma(n+L)}{\prod_{i=1}^L \Gamma(nP_i + 1)} \left(\prod_{i=1}^{L-1} (P'_i)^{nP_i}\right) \frac{(P'_L)^{nP_1+L-1}}{\prod_{i=1}^{L-1} (nP_1+i)}.
	\end{align}
Using \eqref{eq:starling-inequality}, we have
    \begin{align}
        &\prob{\tilde{P}_1 \leq P'_1, \dots, \tilde{P}_{L-1} \leq P'_{L-1}, \tilde{P}_{L} \geq P'_L} \\
        &\geq \frac{\sqrt{2\pi}(n+L)^{n+L-1/2}\mathrm{e}^{-n-L}}{\prod_{i=1}^L \sqrt{2\pi}\mathrm{e}^{1/6}(nP_i+1)^{nP_i+1/2}\mathrm{e}^{-nP_i-1}}\\
        &\quad ~~~~~ \left(\prod_{i=1}^{L} (P'_i)^{nP_i}\right)  \frac{(P'_L)^{L-1}}{\prod_{i=1}^{L-1} (nP_1+i)}\\
        &= \frac{(P'_L)^{L-1}}{(2\pi)^{\frac{L-1}2}\mathrm{e}^{L/6}} \sqrt{\frac{(n+L)^{2L-1}}{{\prod_{i=1}^{L-1} (nP_L+i)^2 \prod_{i=1}^L (nP_i+1)}}}\\
        &\quad\quad \frac{(n+L)^n}{\prod_{i=1}^{L} (n+1/P_i)^{nP_i}} \prod_{i=1}^L \left(\frac{P'_i}{P_i}\right)^{nP_i}\\
        &\geq \frac{(P'_L)^{L-1}}{\mathrm{e}^{L/6}C_1}(n+L)^{-\frac{L-1}{2}}\exp(-n \KL{\vec{P}}{\vec{P}'}).
    \end{align}
\end{proof}

==> Lemma/E_c_lemma.tex <==
\begin{lem}\label{lem:E_c_lemma}
    Let $t_0$ be 
    \begin{align}
    	t_0 &\geq \frac{1}{2(\Delta^\Condorcet_\mathrm{min})^2}\log (4KC'_1) + \frac{8}{(\Delta^\Condorcet_\mathrm{min})^2}\log (2^{L+2}K) \notag\\
	&\quad+  \frac{1+\sqrt{5}}{2}\frac{L^2}{2(\Delta^\Condorcet_\mathrm{min})^4}\left(\log\left(\frac{1}{(\Delta^\Condorcet_\mathrm{min})^2}\log 4KC'_1 \right)\right)^2.  \label{eq:t_0-def}
    \end{align}
    After pulling all arms $t_0$ times, we have
    \begin{align*}
  		\min_{\vec{n}} \prob{E_c(t; \vec{n})} \geq \frac12.
    \end{align*}  
\end{lem}


==> Lemma/UCB_bound.tex <==
\begin{lem}\label{lem:UCB-bound}
    For all $t>0$ and $C_1$ defined in \eqref{eq:c_1-def}, we have
    \begin{align**}
        \prob{|\hat{B}_i(t) - B_i|\leq \beta_i(t)} \geq 1-\frac{KC_1}{t^3},
    \end{align**}
    where $\hat{B}_i(t)$ is the estimated Borda score in \eqref{eq:estimate-Borda-score} and $\beta_i(t)$ is the confidence width in \eqref{eq:Borda-confidence-width} at $t$-th round.
\end{lem}


\begin{proof}[Proof of Lemma~\ref{lem:UCB-bound}]
    Let $\beta'_i(t)=\sqrt{\frac{3\log t + L\log T_i(t)}{2T_i(t)}}$. Since Pinkser's inequality and union bound, we have
    \begin{align*}
        \prob{\forall i\in[K], \left|\hat{\vec{P}}^{(i)}(t) - \vec{P}\right| \leq \beta'_i(t)}
         & \leq 1-\sum_{i=1}^K \prob{\left|\hat{\vec{P}}^{i}(t) - \vec{P}\right| \geq \beta'_i(t)}\\
         & \leq 1-\sum_{i=1}^K \prob{\KL{\hat{\vec{P}}^{i}(t)}{\vec{P}} \geq \frac{3\log t + L\log T_i(t)}{T_i(t)}}\\
         & \leq 1-\sum_{i=1}^K C_1\power{T_i(t)}{L}\exp\left(-(3\log t + L\log T_i(t))\right)\\
         & \leq 1-\frac{C_1K}{t^3}.
    \end{align*}
    The last inequality holds for Lemma~\ref{lem:multinomial-bound}. Given that $\left|\hat{\vec{P}}^{(i)}(t) - \vec{P}\right| \leq \beta'_i(t)$ holds for all $i\in[K]$, we have
    \begin{align*}
        |\hat{B}_i(t) - B_i| &\leq \frac{1}{K-1}\left|\sum_{k\in[K]\backslash\{i\}} \mu(\hat{\vec{P}}^{(i)}(t),\hat{\vec{P}}^{(k)}(t)) - \mu(\vec{P}^{(i)},\vec{P}^{(k)}) \right|\\
        &\leq \frac{1}{K-1}\sum_{k\in[K]\backslash\{i\}} \left|\mu(\hat{\vec{P}}^{(i)}(t),\hat{\vec{P}}^{(k)}(t)) - \mu(\vec{P}^{(i)},\vec{P}^{(k)}) \right|\\
        &\leq \frac{1}{K-1}\sum_{k\in[K]\backslash\{i\}} \left|\mu(\hat{\vec{P}}^{(i)}(t),\hat{\vec{P}}^{(k)}(t)) - \mu(\vec{P}^{(i)},\hat{\vec{P}}^{(k)}(t)) \right| \\
        &\qquad + \left|\mu(\vec{P}^{(i)},\hat{\vec{P}}^{(k)}(t)) - \mu(\vec{P}^{(i)},\vec{P}^{(k)}) \right|\\
        &\leq \frac{1}{K-1}\sum_{k\in[K]\backslash\{i\}} \beta'_i(t) + \beta'_k(t)\\
        &=  \beta'_i(t) +\frac{1}{K-1}\sum_{k\in[K]\backslash\{i\}} \beta'_k(t) = \beta_i(t).
    \end{align*}
    Therefore, we get
    \begin{align*}
        \prob{|\hat{B}_i(t) - B_i|\leq \beta_i(t)} \geq 1-\frac{KC_1}{t^3}.
    \end{align*}
\end{proof}

==> Lemma/multinomial_inf_bound.tex <==
\begin{lem}[Dvoretzky-Kiefer-Wolfowitz inequality] 
    For $\vec{P}, \hat{\vec{P}}$ defined in Lemma~\ref{lem:multinomial-bound}, we have
    \begin{align*}
        \prob{\|\hat{\vec{P}}-\vec{P}\|_\infty \geq \varepsilon} \leq 2 \exp(-2n\varepsilon^2),
    \end{align*}
    for any $\varepsilon>0$ and maximum norm $\|\vec{x}\|_\infty$.
\end{lem}
\begin{proof}
See \cite{Massart1990} for the proof.
\end{proof}

==> Lemma/old_thompson_sub_bound-3-2.tex <==
\begin{lem}\label{lem:thompson_sub_bound-3}
If $t_0$ satisfies condition \eqref{eq:t_0-def} and 
\begin{align}
t_0 &\geq  \frac{1}{2(\Delta'_\mathrm{min})^2}\log (8C'_1) + \frac{8}{(\Delta'_\mathrm{min})^2}\log (2^{L+3}) \\
	&\quad+  \frac{1+\sqrt{5}}{2} \frac{L^2}{2(\Delta'_\mathrm{min})^4}\left(\log\left(\frac{1}{(\Delta'_\mathrm{min})^2}\log 8C'_1 \right)\right)^2 \label{eq:t_0-def-2},
\end{align}
we have
    \begin{align}
    	&\sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t)}\\
	&\quad \leq  \frac{4}{(\Delta'_\mathrm{min})^2} + \frac{C'_1L!}{2^L(\Delta'_\mathrm{min})^{2L}},
    \end{align}
    where $\Delta'_\mathrm{min} = \min_{i\neq a^*_\Condorcet} \frac12 - \mu(\vecarm{y}{i},\vecarm{P}{a^*_\Condorcet})$. 
\end{lem}
\
\begin{proof}
We first define the following events.
\begin{align}
	&\arm{E}{i}_M(t) = \left\{\forall j\neq i,a^*_\Condorcet~~~ \mu(\vecarm{\theta}{i},\vecarm{\theta}{j}) \geq \frac12\right\} \\
	&E_D(t) = \left\{|\vecarm{\theta}{a^*_\Condorcet}-\vecarm{P}{1}| \geq 2\Delta'_{\mathrm{min}} \right\}. \\
\end{align}
Then, we have
\begin{align}
	 &\prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), E_N(t;\vec{n})}\\
	 &\leq \mathbb{P}\left[\mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i})\leq \frac12 , \arm{E}{i}_M(t),\right.\\
	 &\quad \quad \quad~~~~ \left. \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &\leq  \mathbb{P}\left[E_D(t) , \arm{E}{i}_M(t),\right.\\
	 &\quad \quad \quad~~~~\left.\arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &= \mathbb{P}\left[E_D(t), E_N(t;\vec{n}) \bigmid E_c(t;\vec{n})\right]\\
	 &\quad~~~~~~\mathbb{P}\left[\arm{E}{i}_M(t),\arm{E}{i}_P(t), \arm{E}{i}_\theta(t) \bigmid E_c(t;\vec{n})\right]
\end{align}
And,
\begin{align}
	 &\prob{a_t = 1, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), E_N(t;\vec{n})}\\
	 &= \mathbb{P}\left[\forall j \neq a^*_\Condorcet~\mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{j})\geq \frac12 ,\right.\\
	 &\quad \quad \quad~~~~~~~~~~ \left. \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &\geq \mathbb{P}\left[\forall j \neq a^*_\Condorcet~\mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{j})\geq \frac12 ,\right.\\
	 &\quad \quad \quad~ \left.  \arm{E}{i}_M(t), \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &= \mathbb{P}\left[\mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i})\geq \frac12 ,\right.\\
	 &\quad \quad \quad~~~ \left.  \arm{E}{i}_M(t), \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &\geq  \mathbb{P}\left[\overline{E_D(t)} , \arm{E}{i}_M(t),\right.\\
	 &\quad \quad \quad~~~~~\left.\arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})\bigmid E_c(t;\vec{n})\right]\\
	 &= \prob{\overline{E_D(t)}, E_N(t;\vec{n}) \bigmid E_c(t;\vec{n})}\\
	 &\quad~~~~~~\prob{\arm{E}{i}_M(t),\arm{E}{i}_P(t), \arm{E}{i}_\theta(t) \bigmid  E_c(t;\vec{n})}.
\end{align}
Furthermore, from Lemma~\ref{lem:E_c_lemma}, we have
\begin{align}
	 &\prob{\overline{E_D(t)}, E_N(t;\vec{n}) \bigmid E_c(t;\vec{n})}\\
	 &\leq 2\prob{\overline{E_D(t)}, E_N(t;\vec{n}),  E_c(t;\vec{n})} \\
	 &\leq 2\prob{\overline{E_D(t)}, N_1(t) = n_1}.
\end{align}
Therefore, 
\begin{align}
&\prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})}\\
& \leq \frac{\prob{E_D(t), E_N(t;\vec{n}) \bigmid E_c(t;\vec{n})}}{1-\prob{E_D(t), E_N(t;\vec{n}) \bigmid E_c(t;\vec{n})}} \\
&~~~~~~~~~~~~~~~\prob{a_t = 1, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})}\\
&\leq \frac{2\prob{E_D(t), N_1(t)=n_1}}{1-2\prob{E_D(t), N_1(t)=n_1}}\\
&~~~~~~~~~~~~~~~\prob{a_t = 1, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t;\vec{n})}.
\end{align}
From \eqref{eq:t_0-def-2}, we have
\begin{align}
	&\prob{|\vecarm{\theta}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet} | \leq \Delta'_\mathrm{min}} \leq \frac18, \\
	&\prob{|\vecarm{P}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet} | \leq \Delta'_\mathrm{min}} \leq \frac18
\end{align}
from Lemma~\ref{lem:multinomial-l1-bound} and Corollary~\ref{cor:Dirichlet-bound}. Hence,
\begin{align}
	&\mathbb{P}\left[E_D(t), N_{a^*}(t) = n\right]\\
	&\leq \prob{|\vecarm{\theta}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet} | \leq \Delta'_\mathrm{min}, N_1(t) = n_1} \\
	&\quad +\prob{|\vecarm{P}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet} | \leq \Delta'_\mathrm{min}, N_1(t) = n_1} \\
	&\leq \frac18 + \frac18 = \frac14
\end{align}
where the last inequality holds for Lemma~\ref{lem:multinomial-l1-bound} and Corollary~\ref{cor:Dirichlet-bound}. Therefore, if we denote $\prob{E_D(t),N_1(t) = n_1}$ as $p_{n_1}(t) = \prob{E_D(t),N_1(t) = n_1}$, we have
\begin{align}
	&\sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t)}\\
	&\sum_{t=Kt_0}^T\sum_{n_1\dots,n_K}  \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), E_N(t;\vec{n})}\\
	&\leq \sum_{t=Kt_0}^T \sum_{n_1\dots,n_K} \frac{2p_{n_1}(t)}{1-2p_{n_1}(t)}\\
	&\quad ~~~~~~~~~~~~~\prob{a_t = 1, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), E_N(t;\vec{n})}\\
	&\leq \sum_{t=Kt_0}^T\sum_{n_1=t_0}^T \expect{\frac{2p_{n_1}(t)}{1-2p_{n_1}(t)} \indi{a_t = 1, N_1(t)=n_1}}\\
	&\leq \sum_{n_1=t_0}^T \expect{\frac{2p_{n_1}(t)}{1-2p_{n_1}(t)} \indi{a_t = 1, N_1(t)=n_1}}\\
	&\leq \sum_{n_1=t_0}^T 2^{L+1}\exp\left(-\frac12 n_1 (\Delta'_\mathrm{min})^2\right) \\
	&\quad~~~~~~~~~~~~~~~~~+ 2C'_1n_1^L\left(-2 n_1 (\Delta'_\mathrm{min})^2\right)\\
	&\leq  \frac{2^{L+2}}{(\Delta'_\mathrm{min})^2} + \frac{C'_1L!}{2^L(\Delta'_\mathrm{min})^{2L}}
\end{align}

\end{proof}


==> Lemma/old_thompson_sub_bound-3.tex <==
\begin{lem}\label{lem:thompson_sub_bound-3}
If $N_i(Kt_0) = t_0$ for all $i\in[K]$, we have
    \begin{align}
    	&\sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t)}\\
	&\quad \leq  (2^L+C_1)K!\left(\frac{16K}{(\Delta^\Condorcet_\mathrm{min})^2}\right)^K + \frac{16(2^L+C_1)}{(\Delta'_i)^4},
    \end{align}
    where $\Delta'_i = \frac12 - \mu(\vecarm{y}{i},\vecarm{P}{a^*_\Condorcet})$. 
\end{lem}

\begin{proof}
We decompose the probability as follows.
\begin{align*}
&\prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t)}\\
& =  \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \leq \frac{t}{2}}\\
&\quad + \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \geq \frac{t}{2}}.
\end{align*}
From Lemma~\ref{lem:Condorcet_pulled}, we have
\begin{align*}
& \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \leq \frac{t}{2}}\\
&\leq 1- \prob{a_t = a^*_\Condorcet,  N_{a^*_\Condorcet}(t) \leq \frac{t}{2}} \\
&\leq (2^L+C_1)Kt^K\exp\left(-\frac{t}{2K}\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right).
\end{align*}

For the other term, we have
\begin{align}
    &\!\prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \geq \frac{t}{2}}\\
    &=\sum_{n_1,\dots, n_K} \indi{n_{a^*_\Condorcet} \geq \frac{t}{2}}\\
    &\quad~~~~~~~~~~~ \prob{a_t = i,\arm{E}{i}_P(t), \arm{E}{i}_\theta(t), E_N(t; \vec{n})}\\
    &= \sum_{n_1,\dots, n_K} \frac{1}{\prob{E_c(t; \vec{n})}} \indi{n_{a^*_\Condorcet} \geq \frac{t}{2}} \\
    &\quad \prob{\forall j\neq i~\mu(\vecarm{\theta}{i},\vecarm{\theta}{j}) \geq \frac12, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t),E_N(t; \vec{n})}
\end{align}
Since we have $\arm{E}{i}_P(t), \arm{E}{i}_\theta(t)$, $\mu(\vecarm{\theta}{i},\vecarm{\theta}{a^*_\Condorcet})$ is bounded as $\mu(\vecarm{\theta}{i},\vecarm{\theta}{a^*_\Condorcet}) \leq \mu(\vecarm{y}{i},\vecarm{\theta}{a^*_\Condorcet})$ from the definition of $\vecarm{y}{i}$. Therefore, from Lemma~\ref{lem:characters-of-mu},  we need $|\vecarm{\theta}{a^*_\Condorcet} - \vecarm{P}{a^*_\Condorcet}| \geq 2\Delta'_i$ in order to have $\mu(\vecarm{\theta}{i},\vecarm{\theta}{a^*_\Condorcet})\geq \frac12$. Hence,
\begin{align}
    &\!\prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \geq \frac{t}{2}}\\
    &\leq \sum_{n_1,\dots, n_K}  \frac{1}{\prob{E_c(t; \vec{n})}} \indi{n_{a^*_\Condorcet} \geq \frac{t}{2}}\\
    &\quad\quad~~~~~~ \prob{|\vecarm{\theta}{a^*_\Condorcet} - \vecarm{P}{a^*_\Condorcet}| \geq 2\Delta'_i, E_N(t; \vec{n})}\\
    &\leq 2\hspace{-0.3cm}\sum_{n_{a^*_\Condorcet} \geq \frac{t}2} \hspace{-0.3cm}\prob{|\vecarm{\theta}{a^*_\Condorcet} - \vecarm{P}{a^*_\Condorcet}| \geq 2\Delta'_i, N_{a^*_\Condorcet}(t) = n_{a^*_\Condorcet}}.
\end{align}
The last inequality holds for Lemma~\ref{lem:E_c_lemma}.
Now, we bound the probability as 
\begin{align}
 &\prob{|\vecarm{\theta}{a^*_\Condorcet} - \vecarm{P}{a^*_\Condorcet}| \geq 2\Delta'_i, N_{a^*_\Condorcet}(t) = n_{a^*_\Condorcet}}\\
 &\leq  \prob{|\vecarm{P}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet}(t)| \geq \Delta'_i, N_{a^*_\Condorcet}(t) = n_{a^*_\Condorcet}}\\
 &\quad + \prob{|\vecarm{\theta}{a^*_\Condorcet} - \arm{\hat{\vec{P}}}{a^*_\Condorcet}(t)| \geq \Delta'_i, N_{a^*_\Condorcet}(t) = n_{a^*_\Condorcet}}\\
 &\leq (2^L+C_1) \exp\left(-\frac{(\Delta'_{i})^2}{2}n_{a^*_\Condorcet}\right),
\end{align}
where the last inequality holds for Lemma~\ref{lem:multinomial-l1-bound} and Corollary~\ref{cor:Dirichlet-bound}. 
Therefore, 
\begin{align}
    	&\sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t)}\\
	&\leq \sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \leq t/2}\\
	& \quad + \sum_{t=Kt_0}^T \prob{a_t = i, \arm{E}{i}_P(t), \arm{E}{i}_\theta(t), N_{a^*_\Condorcet}(t) \geq t/2}\\
	&\leq \sum_{t=Kt_0}^T (2^L+C_1)Kt^K\exp\left(-\frac{t}{2K}\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right)\\
	& \quad + \sum_{t=Kt_0}^T \sum_{n_{a^*_\Condorcet}=t/2}^t 2(2^L+C_1) \exp\left(-\frac{(\Delta'_{i})^2}{2}n_{a^*_\Condorcet}\right).\\
	&\leq (2^L+C_1)K!\left(\frac{16K}{(\Delta^\Condorcet_\mathrm{min})^2}\right)^K\\
	&\quad + \sum_{t=Kt_0}^T \frac{4(2^L+C_1)}{(\Delta'_i)^2}  \exp\left(-\frac{(\Delta'_{i})^2}{4} t\right)\\
	&\leq (2^L+C_1)K!\left(\frac{16K}{(\Delta^\Condorcet_\mathrm{min})^2}\right)^K + \frac{16(2^L+C_1)}{(\Delta'_i)^4}
    \end{align}

\end{proof}


\begin{comment}
\begin{proof}
	Let $L_i$ be $L_i = (1+\varepsilon)\frac{1}{\KL{\vecarm{P}{i}}{\vecarm{P^*}{i}}}\log T$. If $n_i \geq L_i$ and $t_0 \geq \frac{8}{(\Delta^\Condorcet_\mathrm{min})^2}\log(2K(2^L+C_1))$, we have
\begin{align}
&\!\prob{a_t = i, E^P_i(t), \overline{E^\theta_i(t)}, N_i=n_i}\\
&\leq \prob{a_t = i, \overline{E^\theta_i(t)}, N_i=n_i}\\
&= \hspace{-0.5cm}\sum_{n_1,\dots,n_{i-1},n_{i+1},\dots,n_K} \hspace{-1cm}\prob{a_t = i, \overline{E^\theta_i(t)}, E_N(t; \vec{n})}\\
&\leq \hspace{-0.5cm}\sum_{n_1,\dots,n_{i-1},n_{i+1},\dots,n_K} \hspace{-1cm}\frac{\prob{j\neq i ~ \mu(\vecarm{\theta}{i},\vecarm{\theta}{j})\geq \frac12,  \overline{E^\theta_i(t)}, E_N(t; \vec{n})}}{\prob{E_c(t; \vec{n})}}\\
&\leq \hspace{-0.5cm}\sum_{n_1,\dots,n_{i-1},n_{i+1},\dots,n_K} \hspace{-1cm} 2\prob{ \overline{E^\theta_i(t)}, E_N(t; \vec{n})} \quad(\because \text{Lemma~\ref{lem:E_c_lemma}})\\
&= 2\prob{ \overline{E^\theta_i(t)}, N_i(t) = n_i}\\
&= \frac{2C_1}{T} \quad(\because \text{Lemma~\ref{lem:Event_lemma}}, n_i \geq L_i).
\end{align}
Therefore, 
\begin{align}
    &\sum_{t=K\tau_0}^T \prob{a_t = i, E^P_i(t), \overline{E^\theta_i(t)}}\\
    &\leq \mathbb{E}\left[L_i + \sum_{t=\arm{\tau}{i}_{L_i}}^T \prob{a_t = i, E^P_i(t), \overline{E^\theta_i(t)}}\right] \\
    &\leq \mathbb{E}\left[L_i + \sum_{t=1}^T \frac{2C_1}{T}\right]\\
    &= (1+\varepsilon)\frac{1}{\KL{\vecarm{P}{i}}{\vecarm{P^*}{i}}}\log T+2C_1.
\end{align}
\end{proof}
\end{comment}

==> Proofs/proof_Condorcet_pulled.tex <==
\begin{proof}
From the algorithm, we have
\begin{align*}
	&\prob{a_t \neq a^*_\Condorcet, N_{a^*_\Condorcet}(t) \leq n}\\
	&\leq \prob{\exists i \neq a^*_\Condorcet~\mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \leq \frac12,  N_{a^*_\Condorcet}(t) = n}\\
	&\leq \sum_{n_1,\dots, n_K} \indi{n_{a^*_\Condorcet} \leq n, \sum_{i=1}^K n_i = t}\\
	&\quad \prob{\exists i \neq a^*_\Condorcet~ \mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \leq \frac12,E_N(t;\vec{n})}
\end{align*}
As the same discussion in Lemma~\ref{lem:E_c_lemma}, we have
\begin{align*}
&\prob{\exists i \neq a^*_\Condorcet~ \mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \leq \frac12,E_N(t;\vec{n})}\\
&\leq 1- \prob{\forall i \neq a^*_\Condorcet~ \mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \geq \frac12,E_N(t;\vec{n})}\\
&\leq (2^L+C_1)\sum_{i\in[K]}\exp\left(- n_i\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right).
\end{align*}
Therefore, 
\begin{align*}
	&\prob{a_t = a^*_\Condorcet, N_{a^*_\Condorcet}(t) \leq n}\\
	&\geq \sum_{n_1,\dots, n_K = 1} \indi{n_{a^*_\Condorcet} \leq n, \sum_{i=1}^K n_i = t}\\
	&\quad\quad\quad~~~~~~~~~~\left( \sum_{i \neq a^*_\Condorcet}\exp\left(- n_i\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right)\right)\\
	&\geq 1-(2^L+C_1)Kt^K\exp\left(-\frac{t-n}{K}\frac{(\Delta^\Condorcet_\mathrm{min})^2}{8}\right).
\end{align*}
The last inequality holds for the relationship between arithmetic and geometric mean.
\end{proof}

==> Proofs/proof_E_c_lemma.tex <==
\begin{proof}
	Using Lemma~\ref{lem:characters-of-mu}, we have
	\begin{align*}
		&\prob{E_c(t; \vec{n})}\\
		&\geq \prob{\forall i \neq a^*_\Condorcet ~~ \mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \geq \frac12, E_N(t; \vec{n})}\\
		&\geq \mathbb{P}\left[\forall i \neq a^*_\Condorcet ~~ \left|\vecarm{\theta}{i} - \vecarm{P}{i}\right|\leq \Delta^\Condorcet_i,\right.\\
		&\quad~~~~~~~~~~ \left.\left|\vecarm{\theta}{a^*_\Condorcet} - \vecarm{P}{a^*_\Condorcet}\right|\leq \Delta^\Condorcet_\mathrm{min}, E_N(t; \vec{n})\right]\\
		&\geq 1-\sum_{i=1}^K \prob{\left|\vecarm{\theta}{i} - \vecarm{P}{i}\right|\geq \Delta^\Condorcet_\mathrm{min}, N_i(t) = n_i}\\
		&\geq 1-\sum_{i=1}^K \prob{\left|\vecarm{\theta}{i} - \hat{\vec{P}}^{(i)}(t)\right|\geq \frac12\Delta^\Condorcet_\mathrm{min}, N_i(t) = n_i}\\
		&\quad\quad -\sum_{i=1}^K \prob{\left|\hat{\vec{P}}^{(i)}(t) - \vecarm{P}{i}\right|\geq \frac12\Delta^\Condorcet_\mathrm{min}, N_i(t) = n_i},
	\end{align*}
	where $\hat{\vec{P}}^{(i)}(t)$ be  the estimation of probabilities at $t$-th round, defined as $\hat{\vec{P}}^{(i)}(t) = (C_1^{(i)}(t), \dots, C_L^{(i)}(t))^\top / N_i(t)$. After pulling all arms $t_0$ times, we have $n_i > t_0$ for all $i\in[K]$, and thus
\begin{align*}
	&\prob{\left|\vecarm{\theta}{i} - \hat{\vec{P}}^{(i)}(t)\right| \geq \frac12\Delta^\Condorcet_\mathrm{min}, N_i(t) = n_i}\leq \frac{1}{4K}\\
	&\prob{\left|\vecarm{P}{i} - \hat{\vec{P}}^{(i)}(t)\right| \geq \frac12\Delta^\Condorcet_\mathrm{min}, N_i(t) = n_i}\leq \frac{1}{4K}
\end{align*}
holds for  Lemma~\ref{lem:multinomial-l1-bound} and Corollary~\ref{cor:Dirichlet-bound}.
Therefore, we have
	\begin{align*}
		\min_{\vec{n}}\prob{E_c(t; \vec{n})}
		& \geq 1-\sum_{i=1}^K \frac{1}{4K}  -\sum_{i=1}^K \frac{1}{4K}\\
		&= \frac12.
	\end{align*}
\end{proof}

\begin{comment}
Note that $\Delta'_{\mathrm{min}} \leq \Delta^\Condorcet_{\mathrm{min}}$ by definition.
Furthermore, by the similar discussion, we have
	\begin{align*}
		&\prob{E_c(t) | E^P_i(t),E^\theta_i(t)} \\
		&\geq\prob{\left.\forall i \neq a^*_\Condorcet ~~ \mu(\vecarm{\theta}{a^*_\Condorcet},\vecarm{\theta}{i}) \geq \frac12 \right| E^P_i(t),E^\theta_i(t)} \\
		&\geq \prob{\left|\hat{\vec{P}}^{(a^*_\Condorcet)}-\vecarm{\theta}{a^*_\Condorcet}\right|\leq \Delta'_\mathrm{min}}\\
		&\quad\quad\quad\quad \prob{\forall j\neq i,a^*_\Condorcet ~~ \left|\hat{\vec{P}}^{(j)} - \vecarm{\theta}{j}\right|\leq \Delta^\Condorcet_\mathrm{min}}\\
		&\geq 1-\sum_{j\neq i} \prob{\left|\vecarm{\theta}{i} - \hat{\vec{P}}^{(i)}\right|\geq \frac12\Delta'_\mathrm{min}}\\
		&\quad\quad -\sum_{j\neq i} \prob{\left|\hat{\vec{P}}^{(i)} - \vecarm{P}{i}\right|\geq \frac12\Delta'_\mathrm{min}}\\
		&\geq 1-(2^L+C_1)K \exp\left(-\tau_0 \frac{(\Delta'_\mathrm{min})^2}{8}\right) \geq \frac12.
	\end{align*} 
	Here, we use the fact $\Delta^\Condorcet_j \geq \Delta^\Condorcet_\mathrm{min} \geq \Delta'_\mathrm{min}$.
\end{comment}

==> Proofs/proof_borda_score_bound.tex <==
\begin{proof}
We denote $\varepsilon_1$ and $\varepsilon_2$ as 
\begin{align*}
 &\varepsilon_1 = \frac{2\sqrt{n'}}{\sqrt{n'}+\sqrt{n}}\varepsilon,\\
 &\varepsilon_2 = \frac{\sqrt{n}}{\sqrt{n'}+\sqrt{n}}\varepsilon 
\end{align*}
Let assume that $|\arm{\hat{\vec{P}}}{i}(t) - \arm{\vec{P}}{i}|<\varepsilon_1$ and 
    \begin{align*}
        \max_{k\in[L]} \left|\arm{\hat{\vec{w}}}{j}(t) - \arm{\vec{w}}{j} \right| \leq \varepsilon_2
    \end{align*}
holds for all $j\neq i$. Then, we have
\begin{align*}
    \hat{B}_i(t) &= \frac{1}{K-1} \sum_{j\neq i} \mu(\arm{\hat{\vec{P}}}{i}(t),\arm{\hat{\vec{P}}}{j}(t))\\
    &= \frac{1}{K-1} \sum_{j\neq i} (\arm{\hat{\vec{P}}}{i}(t))^\top\arm{\hat{\vec{w}}}{j}(t)\\
    &= \frac{1}{K-1} \sum_{j\neq i}  (\arm{\hat{\vec{P}}}{i}(t))^\top(\arm{\hat{\vec{w}}}{j}(t)-\vecarm{w}{j} + \vecarm{w}{j})\\
    &\leq \varepsilon_2 + \frac{1}{K-1} \sum_{j\neq i} (\arm{\hat{\vec{P}}}{i}(t))^\top \vecarm{w}{j}\\
    &\quad\quad\quad(\because \max_{k\in[L]} \left|\arm{\hat{\vec{w}}}{j}(t) - \arm{\vec{w}}{j} \right| \leq \frac{\varepsilon}{2})\\
    &= \varepsilon_2 +  \frac{1}{K-1} \sum_{j\neq i} \mu(\arm{\hat{\vec{P}}}{i}(t),\arm{\vec{P}}{j})\\
    &= B_i + \varepsilon_2 \\
    &\quad +\frac{1}{K-1} \sum_{j\neq i} \mu(\arm{\hat{\vec{P}}}{i}(t),\arm{\vec{P}}{j}) -\mu(\arm{\vec{P}}{i},\arm{\vec{P}}{j})\\
    &\leq B_i(t) + \frac{\varepsilon}2  + \frac{\varepsilon}2\\
    &\quad\quad\quad(\because |\arm{\hat{\vec{P}}}{i}(t) - \arm{\vec{P}}{i}|<\varepsilon_1, \text{Lemma~\ref{lem:characters-of-mu}})\\
    &= B_i(t) + \varepsilon.
\end{align*}
We can show $ \hat{B}_i(t) \geq B_i(t) - \varepsilon$ in the same way. Therefore, from union bound and Lemmas~\ref{lem:multinomial-l1-bound}~and~\ref{lem:w-bound}, we have
\begin{align*}
&\prob{|B_i-\hat{B}_i(t)| \geq \varepsilon,  N_i(t) = n', \min_j N_j(t) = n} \\
&\leq  \prob{|\vec{P}^i - \hat{\vec{P}}^i| \geq \varepsilon_1} + \sum_{j\neq i} \prob{ \max_{k\in[L]} \left|\arm{\hat{\vec{w}}}{j}(t) - \arm{\vec{w}}{j} \right| \leq \varepsilon_2}\\
&\leq 2^L \exp\left(-\frac12 n \varepsilon^2\right) + (K-1)2\exp\left(-2 n \left(\frac{\varepsilon}{2}\right)^2\right)\\
&\leq  (2^L +2(K-1))\exp\left(- \frac{2nn'}{(\sqrt{n}+\sqrt{n'})^2}\varepsilon^2\right).
\end{align*}
\end{proof}

==> algorithms/thompson_condorcet_algo_desc.tex <==
The entire algorithm is shown in Algorithm~\ref{Thompson_condorcet}. At each round $t$, the algorithm samples  $\vec{\theta}^{(i)}$ from posterior distributions of $\vec{P}^{(i)}$, and pulls the Condorcet winner in $(\vec{\theta}^{(1)}, \dots, \vec{\theta}^{(L)})$. If it does not exist, sample $(\vec{\theta}^{(1)}, \dots, \vec{\theta}^{(L)})$ again.


==> algorithms/thompson_description.tex <==
The algorithm maintains Bayesian posterior distributions for $\vec{P}^{(i)}$ in each arms. We use the Dirichlet distribution $\Dir(\alpha_1,\dots,\alpha_L)$ to model it, which is the convenient choice when considering rewards from categorical distribution. Let $C_k^{(i)} (i\in[K],\,k\in[L])$ be the number of the times that the reward $k\in[L]$ is observed when arm $i\in[K]$ is pulled. If we employ the prior distribution as $\Dir(1,\dots,1)$, then the posterior distribution given observations $\{C^{(i)}_k\}_{k=1}^L$ would be $\Dir(C_1^{(i)}+1,\dots,C_L^{(i)}+1)$. Thompson Sampling utilizes this posterior distribution to decide the next arm to pull.

==> main_txt/Introduction.tex <==
The multi-armed bandit (MAB) problem is the sequential decision making problem that an agent repeatedly chooses one of $K$ arms of a bandit machine. In each round, the agent receives a random reward that depends on the arm being selected, and the goal is to maximize the cumulative rewards. This problem has been extensively studied recently, both from theoretical and practical aspects. From theoretical point of view, it is shown that the agent must tackle the exploration/exploitation dilemma, in other words, the agent has to balance the pulling of arms that were found to yield high rewards in earlier rounds and the selection of arms that have not yet been tested often enough \cite{Lai1985}.

This MAB problem has many applications as well including the fields outside the computer science, such as the design of clinical trial \cite{villar2015}, economics \cite{Rothschild1974}, and crowdsourcing \cite{Zhou2014}. However, in these applications, feedback is often not given in the numerical way.  For example, the severeness of the side-effect of the medicine is reported on a scale such as {\sf No side-effect---Moderate---Severe}, which is qualitative in nature. Considering the sum of such feedback is clearly invalid and may lead to inadequate conclusion. In this paper, we consider such qualitative feedback, in other words, the case where the feedback is sampled from the distribution on totally ordered set.

There are two approaches to deal with such qualitative feedback. The one is quantile-based approach \cite{Szorenyi2015}. They propose the algorithm that figures out the arms with highest $\tau$-quantile of the distribution of feedback, where $\tau$ is specified by the user. Although it is theoretically well-studied, it can be problematic in practice since the setting of $\tau$ is highly subjective and it ignores the differences of arms if it is not set carefully. Consider the case of the clinical trials for testing the side-effect of two types of medicine, medicine A and B, where the severeness is reported on the scale of {\sf No side-effect---Moderate---Severe}. Let assume that both medicine only have $0.01$ probability of causing the side-effect, and medicine A causes {\sf Moderate} side-effect while medicine B causes {\sf Severe} one. Then, we can clearly conclude that medicine A is more preferable, but for any $\tau \geq 0.01$, quantile-based approach treats them as equal since the feedback at $\tau$-quantile is {\sf No side-effect} for both medicines.

Due to this limitation, we follow the second approach to deal with the qualitative feedback, the dueling bandit approach. The dueling bandit problem \cite{Yue2012} is the problem where the agent learn from relative feedback, which is the result of the noisy comparison of two arms. There are a numerous ways of conducting the comparison, including Bradley-Terry model \cite{Yue2012}, and \cite{Busa-Fekete2013} proposed the comparison with the qualitative feedback. Here, the relative feedback is given as ``which arm gets higher qualitative evaluation'', and thus it is highly objective and prone to the bad feedback, which resolves the drawback in the quantile-based approach. Nevertheless, since the dueling bandit problem is originally proposed for general relative feedback, the algorithms studied in the literature does not fully utilize the qualitative feedback.

In this paper, we propose a new dueling bandit algorithm that directly uses the qualitative information. The algorithm achieves the same goal as ordinary dueling bandit algorithms based on comparison based on qualitative feedback. We theoretically and empirically show that our algorithm outperforms existing methods for the dueling bandit problem. This paper is constructed as follows. After reviewing the existing methods for qualitative feedback in detail, we introduce two types of goals in the bandit problem. Then, we propose algorithms for both goals and derive the theoretical guarantee of performances. Finally, we show the empirical results based on real-world data.






==> main_txt/problem_setting.tex <==
In this section, we formulate the qualitative multi-armed bandit. In the standard multi-armed bandit problem, there are $K$ arms associated with real-valued reward distributions $\nu_1,\dots,\nu_K$. At every round $t$, the agent chooses one arm $a_t \in [K] = \{1,\dots,K\}$ and receives an independent reward $r_t \sim \nu_{a_t}$. The goal of the agent is to maximize the expected cumulative rewards.

In the qualitative multi-armed bandit, the agent chooses one arm at every round as well, but the reward distributions $\{\nu_i\}_{i=1}^K$ are not distributions over real-value but over totally ordered set $(\mathcal{L},\preceq)$ \cite{Szorenyi2015}. For simplicity, we assume that $\mathcal{L} = [L]$ and $\preceq$ denotes the ordinary ranking over the numbers. Thus, distributions $\{\nu_i\}_{i=1}^K$ are all categorical distributions, support of which are $[L]$. Note that even though the rewards $r_t$ are nominal, we shall not make use of its nominal values. 

In order to utilize the ordinal information, we introduce the regret based on pairwise comparison, which is originated in the $K$-armed dueling bandit problem \cite{Yue2012}. We  denote $\mu_{i,j},(i,j\in[K])$ as the probability of arm $i$ wins over arm $j$. This is defined as the probability that the reward given by pulling arm $i$ is larger than that given by pulling arm $j$. Formally,
\[\mu_{i,j} = \prob{X_i > X_j} + \frac12 \prob{X_i = X_j},\]
where $X_i$ is the random variable following distribution $\nu_i$. Note that $\mu_{i,j} + \mu_{j,i} = 1$ and $\mu_{i,i} = \frac12$ holds, which makes $\mu_{i,j}$ a sound winning probability. \cite{Yue2012} proposed the model with the winning probabilities defined as the same way when $\nu_i$ is a Gaussian distribution and \cite{Busa-Fekete2013} discussed the same winning probability for partially ordered set $\mathcal{L}$. 

Based on these noisy comparison, the agent attempts to pull the "best arm" as many times as possible.  There are several definitions of "best arm" \cite{Ramamohan2016}, the one most studied is the Condorcet winner \cite{Urvoy2013}, which is defined as the arm that wins all other arms chance of more than $1/2$. Formally, arm $i^*$ is the Condorcet winner if $\mu_{i^*,j} \geq \frac12$ for all $j\neq i^*$. We denote the Condorcet winner as $a^*_{\Condorcet}$, though it does not always exists. Condorcet winner is studied in various literature \cite{Yue2012,Urvoy2013,Komiyama2015,Wu2016}, in which the agent tries to minimize the regret $R^\Condorcet_T$ is defined as $R^\Condorcet_T = \sum_{t=1}^T \Delta_{a_t}^\Condorcet$ for $\Delta_i^\Condorcet = \mu_{a^*_\Condorcet,i} - \frac12$.

Another definition of winner is the Borda winner \cite{Urvoy2013}, which is the arm that most wins over the average of all arms. Here, we calculate the Borda score $B_i = \frac{1}{K-1} \sum_{j\in[K]\backslash\{i\}} \mu_{i,j}$, which is the average of the winning probability agents other arms. The Borda winner $a^*_\Borda$ is defined as the arm with the largest Border score: $a^*_\Borda = \argmax_{i} B_i$. In this case, the goal of the agent is to minimize another regret $R^\Borda_T = \sum_{t=1}^T \Delta_{a_t}^\Borda$ for $\Delta_i^\Borda = B_{a^*_\Borda} - B_i$. Unlike the Condorcet winner, the Borda winner always exists.

Furthermore, we introduce several quantities related to distribution $\nu_i$. We denote $P^{(i)}_k = \prob{X_i = k}$ and $\vec{P}^{(i)} = (P^{(i)}_1, \dots, P^{(i)}_L) \in \mathcal{D}_L$ where $\mathcal{D}_L$ is the set of probability vectors $\mathcal{D}_L = \{\vec{x}\in\mathbb{R}^L | \vec{x} \geq 0,\, \sum_{i=1}^L x_i = 1\}$. Let the function $\mu:\mathcal{D}_L \times \mathcal{D}_L \to \mathbb{R}$ be defined as
\begin{align}
\mu(\vec{x},\vec{y}) = \sum_{k=1}^L x_k \left(\sum_{l=1}^k y_l - \frac12 y_k\right) \label{eq:mu-def}
\end{align}
so that $\mu(\vec{P}^{(i)},\vec{P}^{(j)}) = \mu_{i,j}$.

==> main_txt/related_work.tex <==
%The multi-armed bandit problem aiming for cumulative regret minimization have been intensively studied for many years, and one of the most famous algorithm is Thompson Sampling \cite{Thompson1933}. This is the Bayesian method which utilizes the posterior distribution for the unknown parameters of the reward distributions. Extensive analysis are conducted on this algorithm, and it is showed that the regret of the Thompson Sampling achieves the information-theoretic lower bound \cite{Komiyama2015}. In this paper, we prove that Thompson sampling is still a useful algorithm even if we employ the qualitative feedback.

%is the only work that considers the qualitative feedback . They defined the ``best arm'' as the arm with the highest $\tau$-percentile point in the feedback distribution and proposed the algorithm to find the best arm and pull it as many times as possible. However, the problem the setting of the percentile $\tau$ is difficult and highly subjective, and there are numerous number of ties if the percentile $\tau$ is not set carefully. Therefore, instead of this definition, we employ other definitions of the ``best arm'' discussed in the dueling bandit problem


The first work of handling qualitative feedback through quantile-based approach is \cite{Szorenyi2015}. In the paper, they studied the problem setting of qualitative feedback problem and propose algorithms for both finite-horizon setting and infinite-horizon setting. The following up work 

The dueling bandit problem is first proposed in \cite{Yue2012}, in which the ``best arm'' is defined through noisy pairwise comparisons of arms, and there is a study \cite{Busa-Fekete2013} that considers the case where comparison is made by the ordered qualitative feedback. We follow this definition and improve their algorithm by directly using the information of the qualitative feedback.

There are several definitions of the ``best arm'' in the dueling bandit \cite{Ramamohan2016}, we focus on the Condorcet winner and Borda winner in this paper. The Condorcet winner is defined as the arm which wins with probability more than $\frac12$ for any other arm. It is the most basic definition of the ``best arm'' in the dueling bandit problem, and a number of algorithms are proposed \cite{Yue2012,Urvoy2013,Komiyama2015,Wu2016} for minimizing the regret metric defined based on the winning probability of the pulled arm when compared with the Condorcet winner. We propose a novel algorithm based on Thompson sampling that minimize the same regret metric using the qualitative feedback.

One drawback of the Condorcet winner is that it does not necessarily exists, while the Borda winner always exists. The Borda winner is defined as the arm with the highest average of winning probability to other arms. There are also numerous works \cite{Busa-Fekete2013,Urvoy2013} that address this definitions. Interestingly, all of these works consider the $\delta$-PAC learning problem, which is to output the Borda winner with the probability of more than $1-\delta$ within minimum number of arm pulls. By the trick introduced in \cite{Yue2012}, $\delta$-PAC learning algorithm can be used for regret minimization, though they empirically performs worse. In this research, we propose the algorithm for regret minimization that is not through $\delta$-PAC learning.
